Landauer's principle in the quantum domain

Recent papers discussing thermodynamic processes in strongly coupled quantum systems claim a violation of Landauer's principle and imply a violation of the second law of thermodynamics. If true, this would have powerful consequences. Perpetuum mobiles could be build as long as the operating temperature is brought close to zero. It would also have serious consequences on thermodynamic derivations of information theoretic results, such as the Holevo bound. Here we argue why these claims are erroneous. Correlations occurring in the strongly coupled, quantum domain require a rethink of how entropy, heat and work are calculated. It is shown that a consistent treatment solves the paradox.

==> eptcsdata.tex <==
\providecommand{\event}{S. B. Cooper, E. Kashefi, P. Panangaden (Eds.): Developments in\\ Computational Models (DCM 2010)}
\providecommand{\volume}{26}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{13}
\providecommand{\eid}{2}

